Reciprocal Normalization for Domain Adaptation

Batch normalization (BN) is widely used in modern deep neural networks, which has been shown to represent the domain-related knowledge, and thus is ineffective for cross-domain tasks like unsupervised domain adaptation (UDA). Existing BN variant methods aggregate source and target domain knowledge in the same channel in normalization module. However, the misalignment between the features of corresponding channels across domains often leads to a sub-optimal transferability. In this paper, we exploit the cross-domain relation and propose a novel normalization method, Reciprocal Normalization (RN). Specifically, RN first presents a Reciprocal Compensation (RC) module to acquire the compensatory for each channel in both domains based on the cross-domain channel-wise correlation. Then RN develops a Reciprocal Aggregation (RA) module to adaptively aggregate the feature with its cross-domain compensatory components. As an alternative to BN, RN is more suitable for UDA problems and can be easily integrated into popular domain adaptation methods. Experiments show that the proposed RN outperforms existing normalization counterparts by a large margin and helps state-of-the-art adaptation approaches achieve better results. The source code is available on https://github.com/Openning07/reciprocal-normalization-for-DA.

==> latex/Supple/Details_Officehome.tex <==
\input{latex/tabs/Supplement_OfficeHome}

==> latex/Supple/Details_Visda.tex <==
\input{latex/tabs/Supplement_Visda}

==> latex/Supple/Diff_Layers.tex <==
\input{latex/figs/Supplement_difflayers}

==> latex/Supple/ExtraExperiment.tex <==
% \input{latex/figs/test/channel_matric}
\section{Additional Comparison Results}
\label{sup_sec:AdditionalComparisonResults}
%%%
%% office-home: different normalization
% \input{latex/Supple/Details_Officehome}

%%%
\paragraph{Train and test time(s) comparisons}
We conduct experiments on UDA task Pr $\to$ Rw (Office-Home) with $4$ threads and one Tesla V100 GPU. The backbones are the ResNet-50.
The training time is obtained from the average of the time cost of 10,000 iterations, including forward and backward operations.
The test times are the total time cost of evaluating the whole target domain dataset.
These results are shown in the Table~\ref{spptab:test_time}.
We can observe that the training time cost of RN is more than vanilla BN, AutoDIAL, and DSBN, but less than TN.
On the other hand, the test time cost of RN is very close to the vanilla BN, and also less than other normalization methods, implying that our RN has more advantages in practical applications.
These results demonstrate that our RN achieves better trade-off between the time costs of both train and test phases and simultaneously achieves better performance according to Table.~\ref{subtab:OfficeHome_results}.

%%%
\myparagraph{Results on small-scale dataset}
We conduct additional experiment on another small-scale dataset Office31, where we adopt ResNet-50 as the backbone.
As listed in Table~\ref{tab:Office31_results}, our RN also helps CDAN obtain an improvement of $1.6\%$ on average.
% Besides, CDAN+RN$^\star$, \ie, ResNet-50 + RN + MinENT , achieves lower performance than CDAN. However, RN$^*$ still outperforms the backbone, verifying the RN's ability to structurally align domains.
These results show the effectiveness of our RN.

\input{latex/tabs/Supplement_TestTime}
\input{latex/tabs/Office31_results}

\input{latex/tabs/Supplement_OfficeHome}
\input{latex/tabs/Supplement_alblation}

%%%
\myparagraph{Detailed Results of Comparison} % list the detailed results %($\ie$ on each task or each class)
i) Table~\ref{subtab:OfficeHome_results}: the ablation study experiments of RC and RA of Office-Home; ii) Table~\ref{subtab:ablation_RCRA_OfficeHome}: the comparison of different normalization modules on Office-Home; and iii) Table~\ref{subtab:ResultsOnVisDA2017}: the detailed class-wise accuracy on VisDA-C.
For fair comparison, all the experiments of CDAN+DSBN are conducted without extra pseudo labels or other loss functions. %, and it is predictable that the performance of DSBN is lower due to the negative transfer.
These results help us better understand the effectiveness of our RN and conduct a better comparison between other counterparts.

\myparagraph{Training Convergence.}
To illustrate the convergence performance and training stability of our RN, we present the classification accuracy during training on the UDA task Art $\to$ Clipart of Office-Home.
As shown in Figure~\ref{analysis:convergence}, the accuracy curve of DSBN drops due to the negative transfer.
Besides, our RN fast and stably converges to the best accuracy, and achieves the optimal accuracy of over $95\%$ with only $1,000$ training iterations (black dotted line).

\input{latex/figs/Supplement_Analysis}

%%%
%% figure 1
% \input{latex/figs/Supplement_difflayers}
% \myparagraph{Visualization of Different Layers}
% To further support our discussions in \textit{Introduction} of the paper, in Figure~\ref{subfig:difflayers}, we illustrate the domain discrepancy of intermediate layers in ResNet-50 on the other $11$ transfer tasks from Office-Home.
% We also show results of RN on different layers in Table~\ref{subtab:AblationOnEachLayer}, where the best accuracies are achieved when all the layers are equipped with RN.
% Thus, with our RN, domain discrepancy in the intermediate layers do decrease and eventually obtain better classification accuracies on the target domain.
% \input{latex/tabs/Supplement_OfficeHome}

%%%
\section{Theoretical Understanding}
\label{sup_sec:theory}

%% gate visualization
\paragraph{Theoretical Insight}
As Ben~\etal~\cite{ben2010theory} pioneered, 
the learning bound of domain adaptation is
$\mathbf{\varepsilon}_{\Tdomain}(h) \leq \mathbf{\varepsilon}_{\Sdomain}(h) + \frac{1}{2} {d_{\mathcal{H} \Delta \mathcal{H}}(\Sdomain, \Tdomain)} + \lambda$, which bounds the expected risk $\mathbf{\varepsilon}_{\Tdomain}(h)$ of a hypothesis $h$ on the target domain by: 
1) the expected risk of $h$ on the source domain, $\mathbf{\varepsilon}_{\Sdomain}(h)$;
2) the A-distance, ${d_{\mathcal{H} \Delta \mathcal{H}}(\Sdomain, \Tdomain)} = 2(1-2\epsilon)$, a domain-divergence measure, where the $\epsilon$ is the error rate of a domain classifier which is trained to discriminate source and target domains;
3) the risk $\lambda$ of an ideal joint hypothesis $h^*$ for both source and target domains.
As shown in Figures~\ref{analysis:a_distance} and \ref{analysis:lambda}, 
%we also compute both the A-Distance $d_{\mathcal{H} \Delta \mathcal{H}}(\Sdomain, \Tdomain)$ and the expected error $\lambda$ of the ideal joint hypothesis $h^*$ on both source and target domains, which are derived on~\cite{ben2010theory}. 
%of different methods including RN, AutoDIAL, TN, and DSBN on the A $\to$ C. 
we compute A-distance and $\lambda$ on the task of A $\to$ C (Office-Home dataset) with CDAN.
%DSBN achieves lower $\lambda$ but higher A-distance, which indicates that it suffers from negative transfer.
Obviously, RN achieves both lower $d_{\mathcal{H} \Delta \mathcal{H}}(\Sdomain, \Tdomain)$ and $\lambda$.
It verifies that RN obtains better generalization performance.

\myparagraph{Distance of the Nearest Channels Across Domains}
In Table~\ref{tab:channel_dist}, we calculate the distance of any two channels across domains in the last BN in each stage. The four stages denote the four ``layer'' in ResNet-50 with channel numbers as 256, 512, 1024, and 2048, respectively.
The distance is calculated by the equation $d^{(j)} = | \frac{\mu_s^{(j)}}{\sqrt{\sigma_s^{2(j)}}} - \frac{\mu_t^{(j)}}{\sqrt{\sigma_t^{2(j)}}}  |$, where $j$ denotes the $j$-th channel, which is introduced in~\cite{wang2019TN}.
Noting that the source and target domains share the same mean and variance in BN, and we do not calculate the distance across domains.
The goal of RN is to find each channel's compensatory information and then aggregate them.
The compensatory  consists of the information of both the corresponding and non-corresponding channels, where the nearest channels across domains has the largest correlation weight.
Hence, we report the sum of the distances between all pairs of the nearest channels.
%which can be either the corresponding or non-corresponding channels.
The smaller distance means the greater ability to align both corresponding and non-corresponding channels to a certain extent.
We can observe that RN obtains the smallest value, implying the better performance of alignment of RN than other methods.
Besides, among the nearest channels, the proportion of corresponding channel is very small, verifying the misalignment between corresponding channels across domains.

\input{latex/tabs/channel_dist}

\input{latex/tabs/Supplement_Visda}

\input{latex/figs/Supplyment_Gate}
% \input{latex/figs/Theoretical_Insight}
\input{latex/figs/T-sne}

%%%
\section{Additional Visualization}
\label{sup_sec:Visualization}
\paragraph{Visualization of $g$ in RA}
For better understanding of RA, we show  visualization of $g$ in RA on UDA tasks Art $\to$ Clipart of Office-Home. We only show the last RN of each layer (\ie, \textit{bn3} in each layer of ResNet50) due to the page limitation. We refer to each stage as stage 1, 2, 3 and 4 with the channel numbers as 256, 512, 1024 and 2048.
The ``1, 2, 3, 4'' on the abscissa axis denote the source mean, source variance, target mean, and target variance, respectively.
The ordinates denote the values of $g$.
As shown in Figure~\ref{subfig:Gate}, RA %are adaptive to the different transfer tasks and
conducts the domain alignment at the intermediate layers in different ways automatically.
Note that, as the number of channels increases, the weights of gates become smaller, which is consistent with the conclusion that the different transferability in the various layers in ~\cite{yosinski2014transferable}, and ensures the significance of RA. 
Similar observations can also be found in other DA scenarios.

%For CDAN$^{-}$, the gates are usually larger than CDAN except in stage 1. 
%It implies that RA-gates further promote the domain alignment without the domain loss ($\ie$ adversarial loss). 
%Theses results demonstrate that the effect of the structural alignment and our RN does play a auxiliary role for the domain loss to further align domains.
% \input{latex/tabs/Supplement_layers_ablation}

\myparagraph{Feature Visualization.}
To further understand the effectiveness of the proposed RN, we visualize the learned representation spaces of different feature normalization modules: vanilla BN~\cite{ioffe2015BN}, AutoDIAL~\cite{cariucci2017autodial}, DSBN~\cite{chang2019domain}, TN~\cite{wang2019TN}, and the proposed RN.
% We utilize the t-SNE~\cite{tsne}
% Figure~\ref{TSNE} shows the visualization of features in the bottleneck in  by the t-SNE~\cite{tsne}
We leverage t-SNE~\cite{tsne} to visualize the feature representations in the bottleneck layer of ResNet-50.
% The compared methods , which are all trained on the UDA task Art $\to$ Clipart from Office-Home benchmark.
As shown in Figure~\ref{TSNE}, CDAN+DSBN suffers from negative transfer, which is the main reason for the sub-optimal results (see Table~\ref{tab:Office31_results}, Table~\ref{subtab:OfficeHome_results}, and Table~\ref{subtab:ResultsOnVisDA2017}).
We also observe that the source and target representations are aligned better by the models integrated RN, compared with existing normalization counterparts.
It demonstrates that our RN is effective to learn the domain-invariant information.
Meanwhile, the cluster centers of two domains in the same class are closer, indicating that the greater ability of RN to learn the discriminative features.

==> latex/Supple/Gate_visualization.tex <==
\input{latex/figs/Supplyment_Gate}

==> latex/Supple/Method.tex <==
\section{More details about RN}
%%%
\subsection{Motivation}
We re-state the motivation of the proposed Reciprocal Normalization (RN) in a clearer way.
In the context of Unsupervised Domain Adaptation (UDA), there are two drawbacks of Batch Normalization (BN): 1) sharing the same mean and variance in different domains is unreasonable and can result in distortion of distribution and domain-specific knowledge; 
2) BN neglects domain discrepancy and cannot conduct domain alignment explicitly, which can lead to sub-optimal performance of domain alignment.
Several latest feature normalization (AutoDIAL, DSBN, and TN) solve the first problems to some extent but do not handle the second issue well.
To handle the two challenges well, we propose RN: through the reciprocity between source and target statistics, RN encourages the statistics of two domains approach each other progressively and leads to better domain alignment eventually. %resulting that the two domain distributions approaching each other.
% With the help of our RN, the source and target features are normalized separately with initial domain statistics at the beginning of training, and then progressively align the domain information via the adaptive reciprocity.
Besides, given different transferability of features from various layers of CNNs, we propose a simple yet effective adaptive gating mechanism to adjust the reciprocity on different layers in an end-to-end way.

%%%%%%%%%%
\input{latex/figs/Supplement_process}

%%%
\subsection{Detailed Formulation}
Figure~\ref{supfig:process} shows a schematic illustration of the proposed RN.

% We supplement complete and brief information for \textbf{Method}.
\myparagraph{Cross-domain Fully-connected Graph (CFG).}
First, we calculate the statistic information of two domains ($\Sdomain$ and $\Tdomain$), $\mu^\Sdomain, (\sigma^2)^\Sdomain$ and $\mu^\Tdomain, (\sigma^2)^\Tdomain$ on each mini-batch:
\begin{equation}
    \mu_{c} = \frac{\sum_{k,i,j}^{B,H,W} x^{\Sdomain}_{kcij}}{BHW}, \  \sigma_{c}^{2} = \frac{\sum_{k,i,j}^{B,H,W} (x^{\Tdomain}_{kcij} - \mu_{c})^{2}}{BHW}.
\label{speq:mu_and_sigma}
\end{equation}

Then we calculate the distance values between statistics of two domains across different channels:
\begin{equation}
    e_{i,j}^{(\mu)} = -(\mu_{i}^{\Sdomain} - \mu_{j}^{\Tdomain})^{2}, \  e_{i,j}^{(\sigma)} = -((\sigma_{i}^{2})^{\Sdomain} - (\sigma_{j}^{2})^{\Tdomain})^{2}.
\end{equation}
In this way, we construct Cross-domain Fully-connected Graph (CFG) with transferability and relevance of each channel.
Next, we obtain the adjacency matrices of Cross-domain Fully-connected Graphs (CFGs):
$E_{\mu}^{\Sdomain \to \Tdomain}$, $E_{\mu}^{\Tdomain \to \Sdomain}$, $E_{\sigma}^{\Sdomain \to \Tdomain}$, and $E_{\sigma}^{\Tdomain \to \Sdomain}$, where $E_{\mu}^{\Sdomain \to \Tdomain} = (E_{\mu}^{\Tdomain \to \Sdomain})^T$ and $E_{\sigma}^{\Sdomain \to \Tdomain} = (E_{\sigma}^{\Tdomain \to \Sdomain})^T$.
The adjacency matrices are used for the reciprocal projection later.
For practical considerations, when the channel dimension is too large ($\eg$ $> 512$), we adopt the group strategy, akin to ~\cite{wu2018GN}.

Then we normalize $E$s row-by-row with softmax for the correlation matrices $\rho_{\mu}^{\Sdomain \to \Tdomain}$, $\rho_{\mu}^{\Tdomain \to \Sdomain}$,  $\rho_{\sigma}^{\Sdomain \to \Tdomain}$ and $\rho_{\sigma}^{\Tdomain \to \Sdomain}$.
Finally, we compute the projections $\tilde{\mu}^{\Sdomain}$, $\tilde{\mu}^{\Tdomain}$, $\tilde{\sigma}^{\Sdomain}$, and $\tilde{\sigma}^{\Tdomain}$:
\begin{equation}
    \tilde{\mu}^{\Sdomain} = \rho_{\mu}^{\Tdomain \to \Sdomain} \otimes \mu^{\Sdomain}, \quad
    \tilde{\mu}^{\Tdomain} = \rho_{\mu}^{\Sdomain \to \Tdomain} \otimes\mu^{\Sdomain},
\end{equation}
\begin{equation}
    (\tilde{\sigma}^{2})^{\Sdomain} = \rho_{\sigma}^{\Tdomain \to \Sdomain} \otimes (\sigma^{2})^{\Sdomain}, \quad
    (\tilde{\sigma}^{2})^{\Tdomain} = \rho_{\sigma}^{\Sdomain \to \Tdomain} \otimes (\sigma^{2})^{\Tdomain},
\end{equation}
where $\otimes$ denotes the matrix multiplication, and $\tilde{x}^{\Sdomain}$ and $\tilde{x}^{\Tdomain}$ denote the projections \textit{from target to source} and the projections \textit{from source to target}, respectively.
In this way, RN conducts the reciprocity by exploiting the transferability and relevance of different channel.

\myparagraph{Reciprocal Aggregation Gate (RA-gate).}
When source and target domains capture the projection information of each other's domain statistics, we propose the RA-gate to aggregate the captured information and the original domain information adaptively.
Specifically, we introduce the learnable gate parameters $g \in [0,1]^C$:
\begin{equation}
    \mu_{agg}^{\Sdomain} = g_{\mu}^{\Sdomain} \cdot \mu^{\Sdomain} + (1-g_{\mu}^{\Sdomain}) \cdot \tilde{\mu}^{\Sdomain},
\end{equation}
\begin{equation}
    \mu_{agg}^{\Tdomain} = g_{\mu}^{\Tdomain} \cdot \mu^{\Tdomain} + (1-g_{\mu}^{\Sdomain}) \cdot \tilde{\mu}^{\Tdomain},
\end{equation}
\begin{equation}
    (\sigma_{agg}^{2})^{\Sdomain} = g_{\sigma}^{\Sdomain} \cdot (\sigma^{2})^{\Sdomain} + (1-g_{\sigma}^{\Sdomain}) \cdot (\tilde{\sigma}^{2})^{\Sdomain},
\end{equation}  
\begin{equation}
    (\sigma_{agg}^{2})^{\Tdomain} = g_{\mu}^{\Tdomain} \cdot (\sigma^{2})^{\Tdomain} + (1-g_{\mu}^{\Sdomain}) \cdot (\tilde{\sigma}^{2})^{\Tdomain}.
\end{equation}

During training RN keeps running estimates of its aggregated mean and variance of each domain via exponential moving average (EMA), similar to BN. Given the $\mu$ and $\sigma$ of the $(t+1)$-th mini-batch of training data, the estimated mean and variance can be calculated by
\begin{equation}
    \hat{\mu}^{\Sdomain}_{new} = (1 - \alpha) \hat{\mu}^{\Sdomain} + \alpha (\mu_{agg}^{\Sdomain})_{t},
\end{equation}
\begin{equation}
    \hat{\mu}^{\Tdomain}_{new} = (1 - \alpha) \hat{\mu}^{\Tdomain} + \alpha (\mu_{agg}^{\Tdomain})_{t},
\end{equation}
\begin{equation}
    (\hat{\sigma}^{2})^{\Sdomain}_{new} = (1 - \alpha) (\hat{\sigma}^{2})^{\Sdomain} + \alpha (\sigma_{agg}^{2})^{\Sdomain})_{t},
\end{equation}
\begin{equation}
    (\hat{\sigma}^{2})^{\Tdomain}_{new} = (1 - \alpha) ((\hat{\sigma}^{2})^{\Tdomain} + \alpha ((\sigma_{agg}^{2})^{\Tdomain})_{t},
\end{equation}
where $\alpha$ is a hyper-parameter and initialized to $0.1$, and $(\cdot)_{t}$ denotes the statistic information after $t$ training iterations.
This strategy enables RN to utilize the estimated domain statistics directly to normalize the examples without performing extra calculations during the evaluation phase.

%%%%%%%
\input{latex/tabs/Supplement_TestTime}


\myparagraph{Separate Normalization.}
To address the first limitation of BN, we adopt the aggregated domain statistics to normalize the features from two domains, separately:
\begin{equation}
    \tilde{x}_{nc}^{\Sdomain} = \gamma_{c} \bar{x}_{nc}^{\Sdomain} + \beta_{c}, \quad
    \tilde{x}_{nc}^{\Tdomain} = \gamma_{c} \bar{x}_{nc}^{\Tdomain} + \beta_{c},
\end{equation}
\begin{equation}
    \bar{x}_{nc}^{\Sdomain}=\frac{x_{nc}^{\Sdomain}-\mu_{agg,nc}^{\Sdomain}}{\sqrt{(\sigma_{agg, nc}^{2})^{\Sdomain} + \epsilon}}, 
    \
    \bar{x}_{nc}^{\Tdomain}=\frac{x_{nc}^{\Tdomain}-\mu_{agg,nc}^{\Tdomain}}{\sqrt{(\sigma_{agg, nc}^{2})^{\Tdomain} + \epsilon}},
\end{equation}
where $\epsilon$ is a small constant to avoid divide-by-zero.

Overall, as shown in Figure~\ref{supfig:process}, RN calculates the statistics of two domains separately and conducts reciprocity according to the \textit{transferability} and \textit{relevance} of various channel. After CFGs, the original and projection statistics are adaptively aggregated via RA-gate. Finally, the new statistics of two domains are used to normalize source and target features separately for the sake of domain-specific knowledge.

%%%
% \subsection{Flow Diagram }
% \input{latex/secs/3__algorithm}

%%%
\subsection{Computational Complexity}
\paragraph{Theoretical} Our RN has a relatively low computational complexity. For the RN at layer $l$, the amount of introduced parameters is $N_{l}=4C_{l}$, where $C_l$ denotes the number of channels at layer $l$.
In each RN, the computation involves two linear multiplication. %That is, our RN introduces reasonable number of parameters and obtains promising improvement.
During the evaluation, the computational complexity of RN is exactly the same as BN.

\myparagraph{Quantitative}
We compare the classification performance and test time of different methods in Table~\ref{spptab:test_time}. Generally, our RN costs the least test time which is the same as that of BN, whil TN is more \textit{ten times} slower than BN. %although TN does not introduce extra parameters. This maybe because the real-time computation in TN is relative large during evaluation phase.
DSBN also conduct one typical BN operation at evaluation but it needs extra time to judge whether the features come from source or target domains. 
% Particularly, as the amount of data smaller, RN even achieves less test time than BN. 
Therefore, our RN achieves both better performance and less test time, which is significant for industrial applications.
%In practice, we find it is not necessary for the neurons to communicate at all layers. The complexity is further limited by adding our NC block to only a few separate layers.

%%%
\subsection{Descriptions of Code}
In the \textit{CodeAndDataAppendix} of our supplementary material, we upload a complete project in one zip file. \textit{reciprocal\_norm.py} contains detailed implementations of the proposed RN. We also have several \textit{run\_X-Y.sh} shell that shows how to reproduce the performance of the corresponding tasks, $\ie$ X $\to$ Y and Y $\to$ X, from Office-Home dataset.

==> latex/figs/Dynamic_reciprocity.tex <==
\begin{figure}
% \setlength{\abovecaptionskip}{0pt}
% \setlength{\belowcaptionskip}{0pt}
    \centering
    \includegraphics[width=\linewidth]{latex/imgs/Dynamic_reciprocity.pdf}
    \caption{Dynamic Reciprocity}
    \label{fig:dynamic_reciprocity}
    % \vspace{-5mm}
\end{figure}
%$\propto$


==> latex/figs/Supplement_difflayers.tex <==
\begin{figure*}
  \centering
    \begin{minipage}{0.82\linewidth}
        \includegraphics[width=1\linewidth]{latex/imgs/supplement/diff_layers_1.pdf}
    \end{minipage}
    \begin{minipage}{0.82\linewidth}
        \includegraphics[width=1\linewidth]{latex/imgs/supplement/diff_layers_2.pdf}
    \end{minipage}
     \begin{minipage}{\linewidth}
        \includegraphics[width=1\linewidth]{latex/imgs/supplement/diff_layers_3.pdf}
    \end{minipage}
  \caption{Visualization results of domain discrepancy (MMD scores) of intermediate layers, $\ie$ the four stages in ResNet-50, on the other $11$ transfer tasks (except A $\to$ C) on Office-Home.}
	\label{subfig:difflayers}
% 	\vspace{0.2in}
\end{figure*}

==> latex/figs/Supplement_process.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{latex/imgs/supplement/process.pdf}
    \caption{A schematic illustration of the proposed RN. Implementation details in training (\textit{left}) and evaluation (\textit{right}).}
    \label{supfig:process}
    \vspace{-5mm}
\end{figure}

==> latex/figs/Theoretical_Insight.tex <==
\begin{figure}%[htb]
  \label{fig:analysis}
% \setlength{\abovecaptionskip}{0pt}
% \setlength{\belowcaptionskip}{0pt}
  \centering
     \subfigure[A-distance]{
     \label{analysis:a_distance}
    %  \begin{minipage}{0.472\linewidth}
            \includegraphics[width=0.46\linewidth]{latex/imgs/compare_ablation/A_distance.png}
        %  \end{minipage}
         }
    \subfigure[lambda]{
        \label{analysis:lambda}
        %  \begin{minipage}{0.472\linewidth}
            \includegraphics[width=0.473\linewidth]{latex/imgs/compare_ablation/Lambda.png}
        %  \end{minipage}
         }
    \label{analysis:theoretical}
    \caption{Theoretical Analysis: A-distance and $\lambda$}.
    \vspace{-3mm}
\end{figure}

==> latex/figs/analysis.tex <==
\begin{figure*}%[htb]
  \label{fig:analysis}
% \setlength{\abovecaptionskip}{0pt}
% \setlength{\belowcaptionskip}{0pt}
  \centering
    \subfigure[]{
        \label{analysis:ablation}
         \begin{minipage}{0.24\linewidth}
            \includegraphics[width=1\linewidth]{latex/imgs/compare_ablation/ablation.pdf}
     \end{minipage}
     }
     \subfigure[]{
     \label{analysis:RA-Gate}
     \begin{minipage}{0.24\linewidth}
            \includegraphics[width=1\linewidth]{latex/imgs/compare_ablation/RA-Gate.pdf}
         \end{minipage}
         }
    \subfigure[]{
    \label{analysis:distance}
    \begin{minipage}{0.225\linewidth}
        \includegraphics[width=1\linewidth]{latex/imgs/compare_ablation/l1_l2_cos.pdf}
    \end{minipage}
    }
    \subfigure[]{
    \label{analysis:convergence}
    \begin{minipage}{0.225\linewidth}
        \includegraphics[width=1\linewidth]{latex/imgs/compare_ablation/convergence.pdf}
    \end{minipage}
    }
%  \subfigure[A-distance]{
%  \label{analysis:a_distance}
%  \begin{minipage}{0.234\linewidth}
%         \includegraphics[width=1\linewidth]{latex/imgs/compare_ablation/A_distance.pdf}
%      \end{minipage}
%      }
% \subfigure[lambda]{
%     \label{analysis:lambda}
%      \begin{minipage}{0.234\linewidth}
%         \includegraphics[width=1\linewidth]{latex/imgs/compare_ablation/Lambda.pdf}
%      \end{minipage}
%      }
    % \label{analysis:distance_and_convergence}
    \caption{(a) The effect of RC and RA. (b) The influence of $g$ in RA. ``L'' means $g$ is learnable. (c) Analysis of the measures of correlations strength in RC (d) Convergence analysis of various feature normalization techniques.}
    \vspace{-3mm}
\end{figure*}

==> latex/figs/analysis2.tex <==
\begin{figure*}%[htb]
  \label{fig:analysis}
% \setlength{\abovecaptionskip}{0pt}
% \setlength{\belowcaptionskip}{0pt}
  \centering
    % \subfigure[]{
    %     \label{analysis:ablation}
    %      \begin{minipage}{0.24\linewidth}
    %         \includegraphics[width=1\linewidth]{latex/imgs/compare_ablation/ablation.pdf}
    %  \end{minipage}
    %  }
     \subfigure[]{
     \label{analysis:RA-Gate}
    %  \begin{minipage}{0.51\linewidth}
            \includegraphics[width=0.48\linewidth]{latex/imgs/compare_ablation/RA-Gate2.pdf}
        %  \end{minipage}
         }
    \subfigure[]{
    \label{analysis:distance}
    % \begin{minipage}{0.45\linewidth}
        \includegraphics[width=0.48\linewidth]{latex/imgs/compare_ablation/l1_l2_cos2.pdf}
    % \end{minipage}
    }
    % \subfigure[]{
    % \label{analysis:convergence}
    % \begin{minipage}{0.225\linewidth}
    %     \includegraphics[width=1\linewidth]{latex/imgs/compare_ablation/convergence.pdf}
    % \end{minipage}
    % }
%  \subfigure[A-distance]{
%  \label{analysis:a_distance}
%  \begin{minipage}{0.234\linewidth}
%         \includegraphics[width=1\linewidth]{latex/imgs/compare_ablation/A_distance.pdf}
%      \end{minipage}
%      }
% \subfigure[lambda]{
%     \label{analysis:lambda}
%      \begin{minipage}{0.234\linewidth}
%         \includegraphics[width=1\linewidth]{latex/imgs/compare_ablation/Lambda.pdf}
%      \end{minipage}
%      }
    % \label{analysis:distance_and_convergence}
    \caption{(a) The influence of $g$ in RA. ``L'' means $g$ is learnable. (b) Analysis of the measures of correlations strength in RC. The backbone is ResNet-50 and the UDA method is CDAN~\cite{long2018CDAN}.}
    \vspace{-3mm}
\end{figure*}

==> latex/figs/channel_visualization.tex <==
\begin{figure*}
  \centering
    $\underbrace{
    \begin{minipage}{0.18\linewidth}
        \includegraphics[width=1\linewidth]{latex/imgs/supplement/gate/A2C_stage1_bn3_noadv.pdf}
    \end{minipage}
    }_{Stage1}$
    % \hspace{-2mm}
   $\underbrace{    
    \begin{minipage}{0.25\linewidth}
        \includegraphics[width=1\linewidth]{latex/imgs/supplement/gate/A2C_stage2_bn3.pdf}
    \end{minipage}
    }_{Stage2}$
   $\underbrace{
     \begin{minipage}{0.37\linewidth}
        \includegraphics[width=1\linewidth]{latex/imgs/supplement/gate/A2C_stage3_bn3.pdf}
    \end{minipage}
    }_{Stage3}$
   $\underbrace{
    \begin{minipage}{0.18\linewidth}
        \includegraphics[width=1\linewidth]{latex/imgs/supplement/gate/A2C_stage4_bn3.pdf}
    \end{minipage}
    }_{Stage4}$

\end{figure*}

==> latex/figs/gate_visualization.tex <==
% \begin{figure}[t]
%   \setlength{\abovecaptionskip}{0pt}
%   \setlength{\belowcaptionskip}{0pt}
%   \centering
%   \subfigure[CDAN+Ours]{
%     \label{analysis:gate_CDAN}
%     \begin{minipage}{0.24\linewidth}
%         \includegraphics[width=1\linewidth]{latex/imgs/R-gate/layer1_2_bn3.pdf}
%     \end{minipage}
%     \begin{minipage}{0.24\linewidth}
%         \includegraphics[width=1\linewidth]{latex/imgs/R-gate/layer2_4_bn3.pdf}
%     \end{minipage}
%     \begin{minipage}{0.24\linewidth}
%         \includegraphics[width=1\linewidth]{latex/imgs/R-gate/layer3_5_bn3.pdf}
%     \end{minipage}
%     \begin{minipage}{0.24\linewidth}
%         \includegraphics[width=1\linewidth]{latex/imgs/R-gate/layer4_2_bn3.pdf}
%     \end{minipage}}
% \subfigure[CDAN$^{-}$+Ours]{
%     \label{analysis:gate_CDAN-}
%      \begin{minipage}{0.24\linewidth}
%         \includegraphics[width=1\linewidth]{latex/imgs/R-gate/layer1_2_bn3_noadv.pdf}
%     \end{minipage}
%     \begin{minipage}{0.24\linewidth}
%         \includegraphics[width=1\linewidth]{latex/imgs/R-gate/layer2_4_bn3_noadv.pdf}
%     \end{minipage}
%     \begin{minipage}{0.24\linewidth}
%         \includegraphics[width=1\linewidth]{latex/imgs/R-gate/layer3_5_bn3_noadv.pdf}
%     \end{minipage}
%     \begin{minipage}{0.24\linewidth}
%         \includegraphics[width=1\linewidth]{latex/imgs/R-gate/layer4_2_bn3_noadv.pdf}
%     \end{minipage}}
%   \caption{Heat-map visualization of R-gates on the adaptation task of A $\to$ C from Office-Home.
%   This ﬁgure is best viewed in the electronic version.}
% 	\label{fig:gate_visualization}
% 	\vspace{-6mm}
% \end{figure}

\begin{figure}
%   \setlength{\abovecaptionskip}{0pt}
%   \setlength{\belowcaptionskip}{0pt}
  \centering
    \label{analysis:gate_CDAN}
    \begin{minipage}{0.24\linewidth}
        \includegraphics[width=1\linewidth]{latex/imgs/R-gate/layer1_2_bn3.pdf}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \includegraphics[width=1\linewidth]{latex/imgs/R-gate/layer2_4_bn3.pdf}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \includegraphics[width=1\linewidth]{latex/imgs/R-gate/layer3_5_bn3.pdf}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \includegraphics[width=1\linewidth]{latex/imgs/R-gate/layer4_2_bn3.pdf}
    \end{minipage}
    \caption{Heat-map visualization of RA-gates on the adaptation task of A $\to$ C from Office-Home. These pictures are best viewed in the electronic version.}
    \label{fig:gate_visualization}
    % \vspace{-3mm}
\end{figure}

==> latex/figs/rn_in_resnet.tex <==
\begin{figure}
\setlength{\abovecaptionskip}{0pt}
\setlength{\belowcaptionskip}{0pt}
    \centering
    \includegraphics[width=0.86\linewidth]{latex/imgs/RN_insert.pdf}
    \caption{RN in the Bottleneck building block presented in ResNets~\cite{he2016resnet}.}
    \label{fig:RN_in_resnet}
    \vspace{-2mm}
\end{figure}

==> latex/figs/test/channel_matric.tex <==
\begin{figure}%[h!]
    \centering
    \includegraphics[width=\linewidth]{latex/imgs/channels/dist_matrix.pdf}
    \caption{Visualization of the quantified transferability of any two channel at the first convolutional layer. The distances between any two channels are computed in the way introduced in~\cite{wang2019TN}(eq.~()), and we choose a Sigmoid gate to normalize the inverse distance to obtain the quantified transferability.}
    \label{fig:transferability_channel}
    \vspace{-5mm}
\end{figure}
%$\propto$

==> latex/macros.tex <==
\usepackage{ifthen}
\definecolor{WeimingColor}{rgb}{0,0,0.8}
\definecolor{XingjiaColor}{rgb}{0.0,0.1,0.9}
\definecolor{FanColor}{rgb}{0.8,0,0.8}
\definecolor{SaulColor}{rgb}{0.8,0.1,0}
\definecolor{YingguoColor}{rgb}{0.0,0.8,0.4}
\definecolor{ZhiyongColor}{rgb}{0.8,0,0.8}

\newcommand{\weiming}[1]{{\color{WeimingColor} [Weiming: #1]}}
\newcommand{\xingjia}[1]{{\color{XingjiaColor}[Xingjia: #1]}}
\newcommand{\saul}[1]{{\color{SaulColor}[Saul: #1]}}
\newcommand{\zhiyong}[1]{{\color{ZhiyongColor}[Zhiyong: #1]}}
\newcommand{\fan}[1]{{\color{FanColor}[Fan: #1]}}
\newcommand{\yingguo}[1]{{\color{YingguoColor}[Yingguo: #1]}}

\newcommand{\warning}[1]{{\it\color{red} #1}}
\newcommand{\toremove}[1]{{\it\color{red} (To remove) #1}}
\newcommand{\note}[1]{{\it\color{blue} #1}}
\newcommand{\nothing}[1]{}

\ifthenelse{\equal{\final}{1}}
{
\renewcommand{\weiming}[1]{}
\renewcommand{\fan}[1]{}
\renewcommand{\xingjia}[1]{}
\renewcommand{\saul}[1]{}
\renewcommand{\zhiyong}[1]{}
\renewcommand{\yingguo}[1]{}

\renewcommand{\warning}[1]{}
\renewcommand{\toremove}[1]{}
\renewcommand{\note}[1]{}
\renewcommand{\nothing}[1]{}
}{}

\hyphenpenalty=1000 % magic number to reduce ugly line breaks

\newcommand{\inputsection}[1]{\input{Sections/#1}}
\newcommand{\inputfigure}[1]{\input{Figures/#1}}
\newcommand{\inputtable}[1]{\input{Tables/#1}}


==> latex/secs/3_algorithm.tex <==
\SetKwComment{Comment}{$\triangleright$\ }{}
\SetCommentSty{itshape}
%%%
\begin{algorithm}[t]
    \DontPrintSemicolon
    \textbf{Input:}  $\{x_{s}, x_{t}\} \in \mathbb{R}^{N \times C \times H \times W}$. \\
    \, \,\qquad Learnable affine parameters: $\gamma$, $\beta$.\\
    % \KwData{$\mu^{s}, (\sigma^{2})^{s}, \mu^{t}, (\sigma^{2})^{t}$}
    \textbf{Output:} {$\widehat{x}_{s}, \widehat{x}_{t}$}\\
    ~\\
    Calculate $\mu_{s}, \mu_{t}, \sigma^2_s, \sigma^2_t$,
    \hfill $ \verb|\\|$  shape:[C, 1] \\
    ~\\
    
    $ E_{t \to s}^{\mu} = -(\mu_{t} - \mu_{s}^T)^2$, \hfill $ \verb|\\|$  shape:[C, C] \\
    $E_{t \to s}^{\sigma^2} = -(\sigma^2_{t} -(\sigma^2_{s})^T)^2,$ 
    \\
    ~\\
    $ E_{s \to t}^{\mu} = (E_{t \to s}^{\mu})^T$, \\
    % \hfill $ \verb|\\|$ \ie, $-(\mu_{s} - \mu_{t}^T)^2$\\
    $E_{s \to t}^{\sigma^2} = (E_{t \to s}^{\sigma^2})^T ,$ \\
    % \hfill $ \verb|\\|$ \ie, $-(\sigma^2_{s} -(\sigma^2_{t})^T)^2$ \\
    ~\\
    Let $z \in \{ \mu, \sigma2 \}$, 
    % \hfill $ \verb|\\|$For concise  expression
    ~\\
    $\rho_{t \to s}^{z} = softmax(E_{t \to s}^{z}, \texttt{dim=1})$, \\
    $\rho_{s \to t}^{z} = softmax(E_{s \to t}^{z}, \texttt{dim=1})$, \\
    ~\\
    % $\rho_{s \to t}^{\mu} = softmax(E_{s \to t}^{\mu}, \texttt{dim=1})$, \\
    % $\rho_{s \to t}^{\sigma^2} = softmax(E_{s \to t}^{\sigma^2}, \texttt{dim=1})$, \\
    % ~\\
    $z_{t, cad} = \rho_{t \to s}^{z} \cdot z_s$, \\
    $z_{s, cad} = \rho_{s \to t}^{z} \cdot z_t$, \\
    ~\\
    $\Tilde{z_t} = g_t^z * z_t + (1-g_t^z) * z_{t, cad}$,\\
    $\Tilde{z_s} = g_s^z * z_s + (1-g_s^z) * z_{s, cad}$,\\  
    ~\\
    % Obtain $\Tilde{\mu_s}, \Tilde{\mu_t}, \Tilde{\sigma^2_s}, and \Tilde{\sigma^2_t}$
    $\widehat{x_s} = \gamma \frac{x_{s}  - \tilde{\mu}_s}{\sqrt{\tilde{\sigma}^{2}_{s} + \epsilon}} + \beta$, \\
    $\widehat{x_t} = \gamma \frac{x_{t}  - \tilde{\mu}_t}{\sqrt{\tilde{\sigma}^{2}_{t} + \epsilon}} + \beta$ \\
    
    Return $\widehat{x_s}, \ \widehat{x_t}$
    \caption{The learning scheme of RN}
    \label{alg:LearningScheme}
\end{algorithm}



==> latex/tabs/DifferentDistances_ablationStudy.tex <==
\begin{table}
    \centering
    \caption{Results of different distance functions on Office-Home benchmark for UDA (ResNet-50).}
    \label{tab:DifferentDistances_ablationStudy}
    \footnotesize{
    \setlength{\tabcolsep}{1.8mm}{
    \begin{tabular}{l|cccc|c}
        \toprule
        Method & Ar$\to$X & Cl$\to$X & Pr$\to$X & Rw$\to$X & AVG \\
        \midrule
        L1 &  &  &  &  &  \\
        L2 &  &  &  &  &  \\
        L2 w/o group &  &  &  &  &  \\
        Cosine &  &  &  &  &  \\
        \bottomrule
    \end{tabular}
    }
    }
\end{table}

==> latex/tabs/DigitFive_MSDA_results.tex <==
\begin{table}
    \centering
    \caption{TODO.}
    \label{tab:DigitFive_MSDA_results}
    \small{
    \begin{tabular}{c|ccc|c}
        \toprule
        Method & $\to$ MNIST-M & $\to$ SVHN & $\to$ SYN & AVG \\
        \hline
        \multicolumn{5}{c}{Single Source BEST} \\
        \hline
         &  &  &  &  \\
         &  &  &  &  \\
         &  &  &  &  \\
        \hline
        \multicolumn{5}{c}{Single Source MIX} \\
        \hline
         &  &  &  &  \\
         &  &  &  &  \\
         &  &  &  &  \\
        \hline
        \multicolumn{5}{c}{Multi Source} \\
        \hline
         &  &  &  &  \\
         &  &  &  &  \\
         &  &  &  &  \\
        LtC &  &  &  &  \\
        LtC + Ours &  &  &  &  \\ 
        \bottomrule
    \end{tabular}
    }
\end{table}

==> latex/tabs/DomainNet_results.tex <==
\begin{table*}%[htb]
    \centering
    \caption{Results ($\%$) on DomainNet benchmark using ResNet-34.
    The table has results of one-shot (1 shot) and three-shot (3 shot) setting on four domains.
    For details about number of runs, we mark the first/second with \textbf{bold}/\underline{underline}.
    }
    \label{tab:DomainNet_results}
    \footnotesize{
    \setlength{\tabcolsep}{2.1mm}{
    \begin{tabular}{l|cccccccccccccc|cc}
        \toprule
        \multirow{2}{*}{Method} & \multicolumn{2}{c}{R to C} & \multicolumn{2}{c}{R to P} & \multicolumn{2}{c}{P to C} & \multicolumn{2}{c}{C to S} & \multicolumn{2}{c}{S to P} & \multicolumn{2}{c}{R to S} & \multicolumn{2}{c|}{P to R} & \multicolumn{2}{c}{AVG} \\
            & \scriptsize{1shot} & \scriptsize{3shot} & \scriptsize{1shot} & \scriptsize{3shot} & \scriptsize{1shot} & \scriptsize{3shot} & \scriptsize{1shot} & \scriptsize{3shot} & \scriptsize{1shot} & \scriptsize{3shot} & \scriptsize{1shot} & \scriptsize{3shot} & \scriptsize{1shot} & \scriptsize{3shot} & \scriptsize{1shot} & \scriptsize{3shot} \\
        \hline
        S + T~\cite{ranjan2017l2} & 55.6 & 60.0 & 60.6 & 62.2 & 56.8 & 59.4 & 50.8 & 55.0 & 56.0 & 59.5 & 46.3 & 50.1 & 71.8 & 73.9 & 56.9 & 60.0 \\
        DANN~\cite{ganin2015DANN} & 58.2 & 59.8 & 61.4 & 62.8 & 56.3 & 59.6 & 52.8 & 55.4 & 57.4 & 59.9 & 52.2 & 54.9 & 70.3 & 72.2 & 58.4 & 60.7 \\
        ADR~\cite{saito2017ADR}   & 57.1 & 60.7 & 61.3 & 61.9 & 57.0 & 60.7 & 51.0 & 54.4 & 56.0 & 59.9 & 49.0 & 51.1 & 72.0 & 74.2 & 57.6 & 60.4 \\
        CDAN~\cite{long2018CDAN}   & 65.0 & 69.0 & 64.9 & 67.3 & 63.7 & 68.4 & 53.1 & 57.8 & 63.4 & 65.3 & 54.5 & 59.0 & 73.2 & 78.5 & 62.5 & 66.5 \\
        ENT~\cite{grandvalet2005ENT}     & 65.2 & 71.0 & 65.9 & 69.2 & 65.4 & 71.1 & 54.6 & 60.0 & 59.7 & 62.1 & 52.1 & 61.1 & 75.0 & \underline{78.6} & 62.6 & 67.6 \\
        MME~\cite{saito2019MME}          & \underline{70.0} & \underline{72.2} & \underline{67.7} & \underline{69.7} & \underline{69.0} & \underline{71.7} & \underline{56.3} & \underline{61.8} & \underline{64.8} & \underline{66.8} & \underline{61.0} & \underline{61.9} & \underline{76.1} & 78.5 & \underline{66.4} & \underline{68.9} \\
        \hline
        {Ours} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
        \bottomrule
    \end{tabular}
    }
    }
\end{table*}

==> latex/tabs/Independent_B2N__.tex <==
% \begin{table*}
%     \centering
%     \footnotesize{
%     \setlength{\tabcolsep}{0.8mm}{
%     \caption{Accuracy ($\%$) on Office-Home for ResNet-50-based UDA and PDA methods.}
%     \label{tab:OfficeHome_results}
%     \begin{tabular}{l|cccccccccccc|c}
%         \toprule
%         Method & Ar$\to$Cl & Ar$\to$Pr & Ar$\to$Rw & Cl$\to$Ar & Cl$\to$Pr & Cl$\to$Rw & Pr$\to$Ar & Pr$\to$Cl & Pr$\to$Rw & Rw$\to$Ar & Rw$\to$Cl & Rw$\to$Pr & AVG \\
%         \hline
%         \multicolumn{14}{c}{\textbf{Closed-set UDA}} \\
%         \hline
%         ResNet-50 & 34.9 & 50.0 & 58.0 & 37.4 & 41.9 & 46.2 & 38.5 & 31.2 & 60.4 & 53.9 & 41.2 & 59.9 & 46.1 \\
%         DAN~\cite{long2015DAN} & 43.6 & 57.0 & 67.9 & 45.8 & 56.5 & 60.4 & 44.0 & 43.6 & 67.7 & 63.1 & 51.5 & 74.3 & 56.3 \\
%         JAN~\cite{long2017JAN} & 45.9 & 61.2 & 68.9 & 50.4 & 59.7 & 61.0 & 45.8 & 43.4 & 70.3 & 63.9 & 52.4 & 76.8 & 58.3 \\
%         % DWT~\cite{roy2019DWT} & 50.3 & 72.1 & 77.0 & 59.2 & 69.3 & 70.2 & 58.3 & 48.1 & 77.3 & 69.3 & 53.6 & 82.0 & 65.6 \\
%         CDAN+BSP~\cite{chen2019BSP} & 52.0 & 68.6 & 76.1 & 58.0 & 70.3 & 70.2 & 58.6 & 50.2 & 77.6 & 72.2 & 59.3 & 81.9 & 66.3 \\
%         SymNet~\cite{zhang2019symnet} & 47.7 & 72.9 & 78.5 & 64.2 & 71.3 & 74.2 & 64.2 & 48.8 & 79.5 & 74.5 & 52.6 & 82.7 & 67.6 \\
%         MDD~\cite{zhang2019MDD} & 54.9 & 73.7 & 77.8 & 60.0 & 71.4 & 71.8 & 61.2 & 53.6 & 78.1 & 72.5 & 60.2 & 82.3 & 68.1 \\
%         % otherB &  &  &  &  &  &  &  &  &  &  &  &  &  \\
%         \hline
%         DANN+BN~\cite{ganin2015DANN} & 45.9 & 61.2 & 68.9 & 50.4 & 59.7 & 61.0 & 45.8 & 43.4 & 70.3 & 63.9 & 52.4 & 76.8 & 58.3 \\
%         DANN+TN & 43.5 & 60.9 & 72.1 & 51.0 & 61.5 & 62.5 & 49.6 & 46.8 & 70.4 & 63.7 & 52.2 & 77.9 & 59.3 \\
%         DANN+NVCC & 47.3 & 63.1 & 74.4 & 57.1 & 64.7 & 68.4 & 55.2 & 47.8 & 75.9 & 68.9 & 53.5 & 79.3 & 63.0 \\
%         \hline
%         CDAN+BN~\cite{long2018CDAN} & 50.7 & 70.6 & 76.0 & 57.6 & 70.0 & 70.0 & 57.4 & 50.9 & 77.3 & 70.9 & 56.7 & 81.6 & 65.8 \\
%         CDAN+TN~\cite{wang2019TN} & 50.2 & 71.4 & 77.4 & 59.3 & 72.7 & 73.1 & 61.0 & 53.1 & 79.5 & 71.9 & 59.0 & 82.9 & 67.6 \\
%         CDAN+NVCC & 55.7 & 73.2 & 78.6 & 64.0 & 74.9 & 74.6 & 66.6 & 57.6 & 81.8 & 75.0 & 60.5 & 84.3 & 70.6 \\
%         % other + Ours &  &  &  &  &  &  &  &  &  &  &  &  &  \\
%         % @ 200729, PDA later
%         \hline
%         \hline
%         \multicolumn{14}{c}{\textbf{Partial-set UDA}} \\
%         \hline
%         ResNet-50 & 46.3 & 67.5 & 75.9 & 59.1 & 59.9 & 62.7 & 58.2 & 41.8 & 74.9 & 67.4 & 48.2 & 74.2 & 61.3 \\
%         DANN~\cite{ganin2015DANN} & 35.5 & 48.2 & 51.6 & 35.2 & 35.4 & 41.4 & 34.8 & 31.7 & 46.2 & 47.5 & 34.7 & 49.0 & 40.9 \\
%         IWAN~\cite{zhang2018IWAN} & 53.9 & 54.5 & 78.1 & 61.3 & 48.0 & 63.3 & 54.2 & 52.0 & 81.3 & 76.5 & 56.8 & 82.9 & 63.6 \\
%         SAN~\cite{cao2018SAN} & 44.4 & 68.7 & 74.6 & 67.5 & 65.0 & 77.8 & 59.8 & 44.7 & 80.1 & 72.2 & 50.2 & 78.7 & 65.3 \\
%         ETN~\cite{cao2019ETN} & 52.9 & 78.2 & 83.2 & 70.2 & 69.4 & 77.6 & 69.5 & 50.8 & 81.0 & 76.3 & 54.5 & 82.0 & 70.5 \\
%         AFN~\cite{xu2019AFN} & 58.9 & 76.3 & 81.4 & 70.4 & 73.0 & 77.8 & 72.4 & 55.3 & 80.4 & 75.8 & 60.4 & 79.9 & 71.8 \\
%         % otherF &  &  &  &  &  &  &  &  &  &  &  &  &  \\
%         \hline
%         ETN+Ours & 56.1 & 79.5 & 87.2 & 74.8 & 68.2 & 79.4 & 77.0 & 52.2 & 83.9 & 82.2 & 58.7 & 83.5 & 73.6 \\
%         \bottomrule
%     \end{tabular}
%     } % setlength
%     } % footnotesize
% \end{table*}


% \begin{table*}
%     \centering
%     \footnotesize{
%     \setlength{\tabcolsep}{0.5mm}{
%     \caption{Accuracy ($\%$) on Office-Home for ResNet-50-based UDA and PDA methods.}
%     \label{tab:OfficeHome_results}
%     \begin{tabular}{l|cccccccccccc|c}
%         \toprule
%         Method & Ar$\to$Cl & Ar$\to$Pr & Ar$\to$Rw & Cl$\to$Ar & Cl$\to$Pr & Cl$\to$Rw & Pr$\to$Ar & Pr$\to$Cl & Pr$\to$Rw & Rw$\to$Ar & Rw$\to$Cl & Rw$\to$Pr & AVG \\
%         \hline
%         \multicolumn{14}{c}{\textbf{Closed-set UDA}} \\
%         \hline
%         ResNet-50 & 34.9 & 50.0 & 58.0 & 37.4 & 41.9 & 46.2 & 38.5 & 31.2 & 60.4 & 53.9 & 41.2 & 59.9 & 46.1 \\
%         DAN~\cite{long2015DAN} & 43.6 & 57.0 & 67.9 & 45.8 & 56.5 & 60.4 & 44.0 & 43.6 & 67.7 & 63.1 & 51.5 & 74.3 & 56.3 \\
%         DANN~\cite{ganin2015DANN} & 45.9 & 61.2 & 68.9 & 50.4 & 59.7 & 61.0 & 45.8 & 43.4 & 70.3 & 63.9 & 52.4 & 76.8 & 58.3 \\
%         JAN~\cite{long2017JAN} & 45.9 & 61.2 & 68.9 & 50.4 & 59.7 & 61.0 & 45.8 & 43.4 & 70.3 & 63.9 & 52.4 & 76.8 & 58.3 \\
%         % DWT~\cite{roy2019DWT} & 50.3 & 72.1 & 77.0 & 59.2 & 69.3 & 70.2 & 58.3 & 48.1 & 77.3 & 69.3 & 53.6 & 82.0 & 65.6 \\
%         CDAN~\cite{long2018CDAN} & 50.7 & 70.6 & 76.0 & 57.6 & 70.0 & 70.0 & 57.4 & 50.9 & 77.3 & 70.9 & 56.7 & 81.6 & 65.8 \\
%         CDAN+BSP~\cite{chen2019BSP} & 52.0 & 68.6 & 76.1 & 58.0 & 70.3 & 70.2 & 58.6 & 50.2 & 77.6 & 72.2 & 59.3 & 81.9 & 66.3 \\
%         CDAN+TN~\cite{wang2019TN} & 50.2 & 71.4 & 77.4 & 59.3 & 72.7 & 73.1 & 61.0 & 53.1 & 79.5 & 71.9 & 59.0 & 82.9 & 67.6 \\
%         SymNet~\cite{zhang2019symnet} & 47.7 & 72.9 & 78.5 & 64.2 & 71.3 & 74.2 & 64.2 & 48.8 & 79.5 & 74.5 & 52.6 & 82.7 & 67.6 \\
%         MDD~\cite{zhang2019MDD} & 54.9 & 73.7 & 77.8 & 60.0 & 71.4 & 71.8 & 61.2 & 53.6 & 78.1 & 72.5 & 60.2 & 82.3 & 68.1 \\
%         % otherB &  &  &  &  &  &  &  &  &  &  &  &  &  \\
%         \hline
%         % DANN+TN & 43.5 & 60.9 & 72.1 & 51.0 & 61.5 & 62.5 & 49.6 & 46.8 & 70.4 & 63.7 & 52.2 & 77.9 & 59.3 \\
%         % DANN+NVCC & 47.3 & 63.1 & 74.4 & 57.1 & 64.7 & 68.4 & 55.2 & 47.8 & 75.9 & 68.9 & 53.5 & 79.3 & 63.0 \\
%         % \hline
%         CDAN+Ours & 55.7 & 73.2 & 78.6 & 64.0 & 74.9 & 74.6 & 66.6 & 57.6 & 81.8 & 75.0 & 60.5 & 84.3 & 70.6 \\
%         % other + Ours &  &  &  &  &  &  &  &  &  &  &  &  &  \\
%         % @ 200729, PDA later
%         \hline
%         \hline
%         \multicolumn{14}{c}{\textbf{Partial-set UDA}} \\
%         \hline
%         ResNet-50 & 46.3 & 67.5 & 75.9 & 59.1 & 59.9 & 62.7 & 58.2 & 41.8 & 74.9 & 67.4 & 48.2 & 74.2 & 61.3 \\
%         DANN~\cite{ganin2015DANN} & 35.5 & 48.2 & 51.6 & 35.2 & 35.4 & 41.4 & 34.8 & 31.7 & 46.2 & 47.5 & 34.7 & 49.0 & 40.9 \\
%         IWAN~\cite{zhang2018IWAN} & 53.9 & 54.5 & 78.1 & 61.3 & 48.0 & 63.3 & 54.2 & 52.0 & 81.3 & 76.5 & 56.8 & 82.9 & 63.6 \\
%         SAN~\cite{cao2018SAN} & 44.4 & 68.7 & 74.6 & 67.5 & 65.0 & 77.8 & 59.8 & 44.7 & 80.1 & 72.2 & 50.2 & 78.7 & 65.3 \\
%         ETN~\cite{cao2019ETN} & 52.9 & 78.2 & 83.2 & 70.2 & 69.4 & 77.6 & 69.5 & 50.8 & 81.0 & 76.3 & 54.5 & 82.0 & 70.5 \\
%         AFN~\cite{xu2019AFN} & 58.9 & 76.3 & 81.4 & 70.4 & 73.0 & 77.8 & 72.4 & 55.3 & 80.4 & 75.8 & 60.4 & 79.9 & 71.8 \\
%         % otherF &  &  &  &  &  &  &  &  &  &  &  &  &  \\
%         \hline
%         ETN+Ours & 56.1 & 79.5 & 87.2 & 74.8 & 68.2 & 79.4 & 77.0 & 52.2 & 83.9 & 82.2 & 58.7 & 83.5 & 73.6 \\
%         \bottomrule
%     \end{tabular}
%     } % setlength
%     } % footnotesize
% \end{table*}


%%% without reference
\begin{table*}
    \centering
    \footnotesize{
    \setlength{\tabcolsep}{0.8mm}{
    \caption{Accuracy ($\%$) on Office-Home for ResNet-50-based UDA and PDA methods.}
    \label{tab:OfficeHome_results}
    \begin{tabular}{l|cccccccccccc|c}
        \toprule
        Method & Ar$\to$Cl & Ar$\to$Pr & Ar$\to$Rw & Cl$\to$Ar & Cl$\to$Pr & Cl$\to$Rw & Pr$\to$Ar & Pr$\to$Cl & Pr$\to$Rw & Rw$\to$Ar & Rw$\to$Cl & Rw$\to$Pr & AVG \\
        \hline
        \multicolumn{14}{c}{\textbf{Closed-set UDA}} \\
        \hline
        ResNet-50 & 34.9 & 50.0 & 58.0 & 37.4 & 41.9 & 46.2 & 38.5 & 31.2 & 60.4 & 53.9 & 41.2 & 59.9 & 46.1 \\
        DAN & 43.6 & 57.0 & 67.9 & 45.8 & 56.5 & 60.4 & 44.0 & 43.6 & 67.7 & 63.1 & 51.5 & 74.3 & 56.3 \\
        DANN & 45.9 & 61.2 & 68.9 & 50.4 & 59.7 & 61.0 & 45.8 & 43.4 & 70.3 & 63.9 & 52.4 & 76.8 & 58.3 \\
        JAN & 45.9 & 61.2 & 68.9 & 50.4 & 59.7 & 61.0 & 45.8 & 43.4 & 70.3 & 63.9 & 52.4 & 76.8 & 58.3 \\
        DWT & 50.3 & 72.1 & 77.0 & 59.2 & 69.3 & 70.2 & 58.3 & 48.1 & 77.3 & 69.3 & 53.6 & 82.0 & 65.6 \\
        CDAN+BSP & 52.0 & 68.6 & 76.1 & 58.0 & 70.3 & 70.2 & 58.6 & 50.2 & 77.6 & 72.2 & 59.3 & 81.9 & 66.3 \\
        AFN & 52.0 & 71.7 & 76.3 & 64.2 & 69.9 & 71.9 & 63.7 & 51.4 & 77.1 & 70.9 & 57.1 & 81.5 & 67.3 \\
        SymNet & 47.7 & 72.9 & 78.5 & 64.2 & 71.3 & 74.2 & 64.2 & 48.8 & 79.5 & 74.5 & 52.6 & 82.7 & 67.6 \\
        MDD & 54.9 & 73.7 & 77.8 & 60.0 & 71.4 & 71.8 & 61.2 & 53.6 & 78.1 & 72.5 & 60.2 & 82.3 & 68.1 \\
        \hline
        CDAN+BN & 50.7 & 70.6 & 76.0 & 57.6 & 70.0 & 70.0 & 57.4 & 50.9 & 77.3 & 70.9 & 56.7 & 81.6 & 65.8 \\
        %CDAN+TN & 50.2 & 71.4 & 77.4 & 59.3 & 72.7 & 73.1 & 61.0 & 53.1 & 79.5 & 71.9 & 59.0 & 82.9 & 67.6 \\
        % otherF &  &  &  &  &  &  &  &  &  &  &  &  &  \\
        CDAN+Ours & 55.6 & 72.6 & 78.1 & 65.7 & 74.7 & 74.5 & 66.2 & 57.1 & 82.0 & 75.2 & 60.5 & 84.6 & 70.6 \\
        % @ 200729, PDA later
        \hline
        \hline
        \multicolumn{14}{c}{\textbf{Partial-set UDA}} \\
        \hline
        ResNet-50 & 46.3 & 67.5 & 75.9 & 59.1 & 59.9 & 62.7 & 58.2 & 41.8 & 74.9 & 67.4 & 48.2 & 74.2 & 61.3 \\
        DANN & 35.5 & 48.2 & 51.6 & 35.2 & 35.4 & 41.4 & 34.8 & 31.7 & 46.2 & 47.5 & 34.7 & 49.0 & 40.9 \\
        IWAN & 53.9 & 54.5 & 78.1 & 61.3 & 48.0 & 63.3 & 54.2 & 52.0 & 81.3 & 76.5 & 56.8 & 82.9 & 63.6 \\
        SAN & 44.4 & 68.7 & 74.6 & 67.5 & 65.0 & 77.8 & 59.8 & 44.7 & 80.1 & 72.2 & 50.2 & 78.7 & 65.3 \\
        AFN & 58.9 & 76.3 & 81.4 & 70.4 & 73.0 & 77.8 & 72.4 & 55.3 & 80.4 & 75.8 & 60.4 & 79.9 & 71.8 \\
        % otherF &  &  &  &  &  &  &  &  &  &  &  &  &  \\
        \hline
        ETN+BN & 52.9 & 78.2 & 83.2 & 70.2 & 69.4 & 77.6 & 69.5 & 50.8 & 81.0 & 76.3 & 54.5 & 82.0 & 70.5 \\
        ETN+Ours & 56.1 & 79.5 & 87.2 & 74.8 & 68.2 & 79.4 & 77.0 & 52.2 & 83.9 & 82.2 & 58.7 & 83.5 & 73.6 \\
        \bottomrule
    \end{tabular}
    } % setlength
    } % footnotesize
\end{table*}

==> latex/tabs/Office31_MSDA.tex <==
\begin{table}
    \centering
    \caption{Accuracy (\%) on multi-source domain adaptation on Office-31 benchmark.}
    \label{tab:Office31_Results_MSDA}
    \footnotesize{
    \setlength{\tabcolsep}{1.6mm}{
    \begin{tabular}{l|ccc|c}
        \toprule
        Method & A+D$\to$W & A+W$\to$D & D+W$\to$A & AVG \\
        \hline
        \multicolumn{5}{c}{\textbf{AlexNet~\cite{krizhevsky2012AlexNet}}} \\
        \hline
        AlexNet~\cite{krizhevsky2012AlexNet} & 89.1 & 94.6 & 49.1 & 77.6 \\
        AlexNet+BN~\cite{ioffe2015BN} & 92.9 & 95.2 & 60.1 & 82.7 \\
        % DIAL & 94.3 & 93.8 & 62.5 & 83.5 \\
        AlexNet+DA-layers~\cite{mancini2018DAlayers} & 94.6 & 93.7 & 62.6 & 83.6 \\
        AlexNet+Ours & 95.1 & 96.6 & 61.8 & 84.5 \\
        \hline
        \hline
        \multicolumn{5}{c}{\textbf{ResNet-50~\cite{he2016resnet}}} \\
        \hline
        CDAN(+BN)~\cite{long2018CDAN} &  &  &  &  \\
        CDAN+DSBN~\cite{chang2019domain} & 99.3 & 99.4 & 70.1 & 89.6 \\
        CDAN+Ours & 99.3 & 99.8 & 76.6 & 91.9 \\
        \bottomrule
    \end{tabular}
    }
    }
    % \vspace{-3mm}
\end{table}

==> latex/tabs/Office31_results.tex <==
% \begin{table}
%     \centering\caption{Results ($\%$) on Office-31 for UDA on ResNet-50. Note that results of CDAN+TN, CAN, and X are obtained by running the official implementations.}
%     \label{tab:Office31_results}
%     \footnotesize{
%     \setlength{\tabcolsep}{0.8mm}{
%     \begin{tabular}{l|cccccc|c}
%         \toprule
%         Method & A$\to$W & D$\to$W & W$\to$D & A$\to$D & D$\to$A & W$\to$A & AVG \\
%         \hline
%         ResNet-50 & 68.4 & 96.7 & 99.3 & 68.9 & 62.5 & 60.7 & 76.1 \\
%         DAN~\cite{ganin2015DAN} & 80.5 & 97.1 & 99.6 & 78.6 & 63.6 & 62.8 & 80.4 \\
%         DANN~\cite{ganin2015DANN} & 82.0 & 96.9 & 99.1 & 79.7 & 68.2 & 67.4 & 82.2 \\
%         JAN~\cite{long2017JAN} & 86.0 & 96.7 & 99.7 & 85.1 & 69.2 & 70.7 & 84.6 \\
%         GTA~\cite{sankaranarayanan2018GTA} & 89.5 & 97.9 & 99.8 & 87.7 & 72.8 & 71.4 & 86.5 \\
%         MCD~\cite{saito2018MCD} & 88.6 & 98.5 & 100.0 & 92.2 & 69.5 & 69.7 & 86.5 \\
%         CDAN+BSP~\cite{chen2019BSP} & 93.3 & 98.2 & 100.0 & 93.0 & 73.6 & 72.6 & 88.5 \\
%         DSBN~\cite{chang2019domain} & 92.7 & 99.0 & 100.0 & 92.2 & 71.7 & 74.4 & 88.3 \\
%         CDAN+BNM~\cite{cui2020BNM} & 92.8 & 98.8 & 100.0 & 92.9 & 73.5 & 73.8 & 88.6 \\
%         \hline
%         CDAN+BN~\cite{long2018CDAN} & 94.1 & 98.6 & 100.0 & 92.9 & 71.0 & 69.3 & 87.7 \\
%         CDAN+TN~\cite{wang2019TN} & 95.7 & 98.7 & 100.0 & 94.0 & 73.4 & 74.2 & 89.3 \\
%         CDAN+NVCC & 94.5 & 98.2 & 100.0 & 95.3 & 74.0 & 74.0 & 89.3 \\
%         \bottomrule
%     \end{tabular}
%     }
%     }
% \end{table}

% \begin{table}
%     \centering\caption{Results ($\%$) on Office-31 for UDA on ResNet-50. %Note that results of CDAN+TN, CAN, and X are obtained by running the official implementations.
%     }
%     \label{tab:Office31_results}
%     \footnotesize{
%     \setlength{\tabcolsep}{0.6mm}{
%     \begin{tabular}{l|cccccc|c}
%         \toprule
%         Method & A$\to$W & D$\to$W & W$\to$D & A$\to$D & D$\to$A & W$\to$A & AVG \\
%         \hline
%         ResNet-50 & 68.4 & 96.7 & 99.3 & 68.9 & 62.5 & 60.7 & 76.1 \\
%         DAN~\cite{long2015DAN} & 80.5 & 97.1 & 99.6 & 78.6 & 63.6 & 62.8 & 80.4 \\
%         DANN~\cite{ganin2015DANN} & 82.0 & 96.9 & 99.1 & 79.7 & 68.2 & 67.4 & 82.2 \\
%         JAN~\cite{long2017JAN} & 86.0 & 96.7 & 99.7 & 85.1 & 69.2 & 70.7 & 84.6 \\
%         GTA~\cite{sankaranarayanan2018GTA} & 89.5 & 97.9 & 99.8 & 87.7 & 72.8 & 71.4 & 86.5 \\
%         MCD~\cite{saito2018MCD} & 88.6 & 98.5 & 100.0 & 92.2 & 69.5 & 69.7 & 86.5 \\
%         CRST~\cite{zou2019CRST} & 89.4 & 98.9 & 100.0 & 88.7 & 72.6 & 70.9 & 86.8 \\
%         CDAN~\cite{long2018CDAN} & 94.1 & 98.6 & 100.0 & 92.9 & 71.0 & 69.3 & 87.7 \\
%         CDAN+BSP~\cite{chen2019BSP} & 93.3 & 98.2 & 100.0 & 93.0 & 73.6 & 72.6 & 88.5 \\
%         DSBN~\cite{chang2019domain} & 92.7 & 99.0 & 100.0 & 92.2 & 71.7 & 74.4 & 88.3 \\
%         CDAN+BNM~\cite{cui2020BNM} & 92.8 & 98.8 & 100.0 & 92.9 & 73.5 & 73.8 & 88.6 \\
%         \hline
%         % CDAN+TN~\cite{wang2019TN} & 95.7 & 98.7 & 100.0 & 94.0 & 73.4 & 74.2 & 89.3 \\
%         CDAN+Ours & 94.5 & 98.2 & 100.0 & 95.3 & 74.0 & 74.0 & 89.3 \\
%         \bottomrule
%     \end{tabular}
%     }
%     }
% \end{table}

%%% without reference
\begin{table}
% \setlength{\abovecaptionskip}{0pt}
     \centering\caption{Accuracy ($\%$) on small-scale Office-31 for UDA. %Note that results of CDAN+TN, CAN, and X are obtained by running the official implementations.
    }
    \label{tab:Office31_results}
    \small{
    \setlength{\tabcolsep}{0.8mm}{
    \begin{tabular}{lccccccc}
        \toprule
        Method & A$\to$W & D$\to$W & W$\to$D & A$\to$D & D$\to$A & W$\to$A & AVG \\
        \midrule
        ResNet-50 & 68.4 & 96.7 & 99.3 & 68.9 & 62.5 & 60.7 & 76.1 \\
        %DAN & 80.5 & 97.1 & 99.6 & 78.6 & 63.6 & 62.8 & 80.4 \\
        DANN~\cite{ganin2015DANN} & 82.0 & 96.9 & 99.1 & 79.7 & 68.2 & 67.4 & 82.2 \\
        JAN~\cite{long2017JAN} & 86.0 & 96.7 & 99.7 & 85.1 & 69.2 & 70.7 & 84.6 \\
        MCD~\cite{saito2018MCD} & 88.6 & 98.5 & 100.0 & 92.2 & 69.5 & 69.7 & 86.5 \\
        AFN~\cite{xu2019AFN} & 90.1 & 98.6 & 99.8 & 90.7 & 73.0 & 70.2 & 87.1 \\
        CRST~\cite{zou2019CRST} & 89.4 & 98.9 & 100.0 & 88.7 & 72.6 & 70.9 & 86.8 \\
        iCAN~\cite{zhang2018iCAN} & 92.5 & 98.8 & 100.0 & 90.1 & 72.1 & 69.9 & 87.2 \\
        DMRL~\cite{wu2020dual} & 90.8 & \textbf{99.0} & 100.0 & 93.4 & 73.0 & 71.2 & 87.9 \\
        DSBN~\cite{chang2019domain} & 92.7 & \textbf{99.0} & 100.0 & 92.2 & 71.7 & 74.4 & 88.3 \\
        SymNet~\cite{zhang2019symnet} & 90.8 & 98.8 & 100.0 & 93.9 & 74.6 & 72.5 & 88.4 \\
        BSP~\cite{chen2019BSP} & 93.3 & 98.2 & 100.0 & 93.0 & 73.6 & 72.6 & 88.5 \\
        BNM~\cite{cui2020BNM} & 92.8 & 98.8 & 100.0 & 92.9 & 73.5 & 73.8 & 88.6 \\
        IAA~\cite{jiang2020implicit} & 90.3 & 98.7 & 99.8 & 92.1 & \textbf{75.3} & \textbf{74.9} & 88.8 \\
        CDAN-GD & 93.7 & 94.0 & 98.6 & 100.0 & 73.4 & 73.0 & 88.8 \\
        \midrule
        CDAN~\cite{long2018CDAN} & 94.1 & 98.6 & 100.0 & 92.9 & 71.0 & 69.3 & 87.7 \\
        % CDAN+TN~\cite{wang2019TN} & 95.7 & 98.7 & 100.0 & 94.0 & 73.4 & 74.2 & 89.3 \\
        % +RN$^{\star}$ & 92.8 & 95.5 & 100.0 & 93.8 & 68.1 & 66.5 & 86.1 \\
        CDAN+RN & \textbf{94.5} & 98.2 & \textbf{100.0} & \textbf{95.3} & 74.0 & 74.0 & \textbf{89.3} \\
        \bottomrule
    \end{tabular}
    }
    }
    \vspace{-4mm}
\end{table}

==> latex/tabs/Regularizer_ImageClef.tex <==
% \begin{table}
%     \centering
%     \caption{Accuracy ({\%}) on Image-CLEF-DA \textit{as regularizer} for UDA (ResNet-50).}
%     \label{tab:regularizer_ImageCLEFDA_results}
%     \footnotesize{
%     \setlength{\tabcolsep}{1.6mm}{
%     \begin{tabular}{l|cccccc|c}
%         \toprule
%         Method & I$\to$P & P$\to$I & I$\to$C & C$\to$I & C$\to$P & P$\to$C & AVG \\
%         \hline
%         DANN+BN~\cite{ganin2015DANN} & 75.0 & 86.0 & 96.2 & 87.0 & 74.3 & 91.5 & 85.0 \\
%         DANN+TN~\cite{wang2019TN} & 78.2 & 89.5 & 95.5 & 91.0 & 76.0 & 91.5 & 87.0 \\
%         DANN+NVCC & 78.1 & 90.1 & 96.3 & 91.7 & 78.0 & 94.0 & 88.0 \\ 
%         \hline
%         CDAN+BN ~\cite{long2018CDAN} & 77.7 & 90.7 & 97.7 & 91.3 & 74.2 & 94.3 & 87.7 \\
%         CDAN+TN~\cite{wang2019TN} & 78.3 & 90.8 & 96.7 & 92.3 & 78.0 & 94.8 & 88.5 \\
%         CDAN+NVCC & 78.6 & 92.7 & 96.7 & 92.8 & 79.1 & 94.8 & 89.1 \\
%         \bottomrule
%     \end{tabular}
%     }
%     }
% \end{table}

%%% without reference
\begin{table}[htb]
    \centering
    \caption{Accuracy ({\%}) on Image-CLEF-DA \textit{as regularizer} for UDA (ResNet-50).}
    \label{tab:regularizer_ImageCLEFDA_results}
    \footnotesize{
    \setlength{\tabcolsep}{1.2mm}{
    \begin{tabular}{l|cccccc|c}
        \toprule
        Method & I$\to$P & P$\to$I & I$\to$C & C$\to$I & C$\to$P & P$\to$C & AVG \\
        \hline
        DANN+BN & 75.0 & 86.0 & 96.2 & 87.0 & 74.3 & 91.5 & 85.0 \\
        DANN+TN & 78.2 & 89.5 & 95.5 & 91.0 & 76.0 & 91.5 & 87.0 \\
        DANN+NVCC & 78.1 & 90.1 & 96.3 & 91.7 & 78.0 & 94.0 & 88.0 \\ 
        \hline
        \hline
        CDAN+BN & 77.7 & 90.7 & 97.7 & 91.3 & 74.2 & 94.3 & 87.7 \\
        CDAN+TN & 78.3 & 90.8 & 96.7 & 92.3 & 78.0 & 94.8 & 88.5 \\
        CDAN+NVCC & 78.6 & 92.7 & 96.7 & 92.8 & 79.1 & 94.8 & 89.1 \\
        \bottomrule
    \end{tabular}
    }
    }
\end{table}

==> latex/tabs/Regularizer_OfficeHome.tex <==
% \begin{table*}
%     \centering
%     \footnotesize{
%     \setlength{\tabcolsep}{1.0mm}{
%     \caption{Accuracy ({\%}) on Office-home \textit{as regularizer} for UDA (ResNet-50).}
%     \label{tab:regularizer_OfficeHome_results}
%     \begin{tabular}{l|cccccccccccc|c}
%         \toprule
%         Method & Ar$\to$Cl & Ar$\to$Pr & Ar$\to$Rw & Cl$\to$Ar & Cl$\to$Pr & Cl$\to$Rw & Pr$\to$Ar & Pr$\to$Cl & Pr$\to$Rw & Rw$\to$Ar & Rw$\to$Cl & Rw$\to$Pr & AVG \\
%         % otherB &  &  &  &  &  &  &  &  &  &  &  &  &  \\
%         \hline
%         DANN+BN~\cite{ganin2015DANN} & 45.9 & 61.2 & 68.9 & 50.4 & 59.7 & 61.0 & 45.8 & 43.4 & 70.3 & 63.9 & 52.4 & 76.8 & 58.3 \\
%         DANN+TN & 43.5 & 60.9 & 72.1 & 51.0 & 61.5 & 62.5 & 49.6 & 46.8 & 70.4 & 63.7 & 52.2 & 77.9 & 59.3 \\
%         DANN+NVCC & 47.3 & 63.1 & 74.4 & 57.1 & 64.7 & 68.4 & 55.2 & 47.8 & 75.9 & 68.9 & 53.5 & 79.3 & 63.0 \\
%         \hline
%         CDAN+BN~\cite{long2018CDAN} & 50.7 & 70.6 & 76.0 & 57.6 & 70.0 & 70.0 & 57.4 & 50.9 & 77.3 & 70.9 & 56.7 & 81.6 & 65.8 \\
%         CDAN+TN~\cite{wang2019TN} & 50.2 & 71.4 & 77.4 & 59.3 & 72.7 & 73.1 & 61.0 & 53.1 & 79.5 & 71.9 & 59.0 & 82.9 & 67.6 \\
%         CDAN+NVCC & 55.7 & 73.2 & 78.6 & 64.0 & 74.9 & 74.6 & 66.6 & 57.6 & 81.8 & 75.0 & 60.5 & 84.3 & 70.6 \\
%         % other + Ours &  &  &  &  &  &  &  &  &  &  &  &  &  \\
%         % @ 200729, PDA later
%         \hline
     
%     \end{tabular}
%     } % setlength
%     } % footnotesize
% \end{table*}


%%% without reference
\begin{table*}
    \centering
    \footnotesize{
    \setlength{\tabcolsep}{0.8mm}{
    \caption{Accuracy ({\%}) on Office-home \textit{as regularizer} for UDA (ResNet-50).}
    \label{tab:regularizer_OfficeHome_results}
    \resizebox{0.95\textwidth}{!}{
    \begin{tabular}{l|cccccccccccc|c}
        \toprule
        Method & Ar$\to$Cl & Ar$\to$Pr & Ar$\to$Rw & Cl$\to$Ar & Cl$\to$Pr & Cl$\to$Rw & Pr$\to$Ar & Pr$\to$Cl & Pr$\to$Rw & Rw$\to$Ar & Rw$\to$Cl & Rw$\to$Pr & AVG \\
        % otherB &  &  &  &  &  &  &  &  &  &  &  &  &  \\
        \hline
        DANN+BN & 45.9 & 61.2 & 68.9 & 50.4 & 59.7 & 61.0 & 45.8 & 43.4 & 70.3 & 63.9 & 52.4 & 76.8 & 58.3 \\
        DANN+TN & 43.5 & 60.9 & 72.1 & 51.0 & 61.5 & 62.5 & 49.6 & 46.8 & 70.4 & 63.7 & 52.2 & 77.9 & 59.3 \\
        DANN+NVCC & 47.3 & 63.1 & 74.4 & 57.1 & 64.7 & 68.4 & 55.2 & 47.8 & 75.9 & 68.9 & 53.5 & 79.3 & 63.0 \\
        \hline
        \hline
        CDAN+BN & 50.7 & 70.6 & 76.0 & 57.6 & 70.0 & 70.0 & 57.4 & 50.9 & 77.3 & 70.9 & 56.7 & 81.6 & 65.8 \\
        CDAN+TN & 50.2 & 71.4 & 77.4 & 59.3 & 72.7 & 73.1 & 61.0 & 53.1 & 79.5 & 71.9 & 59.0 & 82.9 & 67.6 \\
        CDAN+NVCC & 55.7 & 73.2 & 78.6 & 64.0 & 74.9 & 74.6 & 66.6 & 57.6 & 81.8 & 75.0 & 60.5 & 84.3 & 70.6 \\
        % other + Ours &  &  &  &  &  &  &  &  &  &  &  &  &  \\
        % @ 200729, PDA later
        \bottomrule
    \end{tabular}
    } % setlength
    } % footnotesize
\end{table*}

==> latex/tabs/Regularizer_VisDA2017C.tex <==
% \begin{table}
%     \centering
%     \caption{Accuracy ({\%}) on VisDA-2017 \textit{as regularizer} for UDA (ResNet-50).}
%     \label{tab:Regularizer_VisDA2017_results}
%     \footnotesize{
%     \setlength{\tabcolsep}{1.6mm}{
%     \begin{tabular}{c|cc}
%         \toprule
%         \multirow{2}{*}{Method} & \multicolumn{2}{c}{Synthetic $\to$ Real} \\
%         \cline{2-3}
%          & ResNet-50 & ResNet-101 \\
%         \hline
%         DANN+BN~\cite{ganin2015DANN} & 63.7 &  \\
%         DANN+TN~\cite{wang2019TN} & 66.3 &  \\
%         DANN+NVCC &  &  \\ 
%         \hline
%         CDAN+BN ~\cite{long2018CDAN} & 70.0 &  \\
%         CDAN+TN~\cite{wang2019TN} & 71.4 &  \\
%         CDAN+NVCC & 74.1 &  \\
%         \bottomrule
%     \end{tabular}
%     }
%     }
% \end{table}


%%% without reference
\begin{table}
\setlength{\abovecaptionskip}{0pt}
    \centering
    \caption{Classification accuracies ({\%}) on VisDA-2017 \textit{as regularizer} for UDA (ResNet-50).}
    \label{tab:Regularizer_VisDA2017_results}
    \scriptsize{
    \setlength{\tabcolsep}{3.6mm}{
    \begin{tabular}{c|cc}
        \toprule
        \multirow{2}{*}{Method} & \multicolumn{2}{c}{Synthetic $\to$ Real} \\
        \cline{2-3}
         & ResNet-50 & ResNet-101 \\
        \hline
        DANN+BN & 63.7 &  \\
        DANN+TN & 66.3 &  \\
        DANN+NVCC &  &  \\ 
        \hline
        CDAN+BN & 70.0 &  \\
        CDAN+TN & 71.4 &  \\
        CDAN+NVCC & 74.1 &  \\
        \bottomrule
    \end{tabular}
    }
    }
\end{table}

==> latex/tabs/Supplement_OfficeHome.tex <==
%% without reference
\begin{table*}
    \centering
    % \setlength{\abovecaptionskip}{0pt}
    % \captionsetup{font={footnotesize}}
    \footnotesize{
    \setlength{\tabcolsep}{0.9mm}{
    \caption{UDA accuracy ($\%$) of different feature normalization methods on Office-Home (ResNet-50).}
    \label{subtab:OfficeHome_results}
    \begin{tabular}{lccccccccccccc}
        \toprule
        Method & Ar$\to$Cl & Ar$\to$Pr & Ar$\to$Rw & Cl$\to$Ar & Cl$\to$Pr & Cl$\to$Rw & Pr$\to$Ar & Pr$\to$Cl & Pr$\to$Rw & Rw$\to$Ar & Rw$\to$Cl & Rw$\to$Pr & AVG \\
        % \midrule
        % \multicolumn{14}{c}{ResNet-50} \\
        \midrule
        ResNet-50 (source only) & 34.9 & 50.0 & 58.0 & 37.4 & 41.9 & 46.2 & 38.5 & 31.2 & 60.4 & 53.9 & 41.2 & 59.9 & 46.1 \\
        \midrule
        DANN(+BN) & 45.9 & 61.2 & 68.9 & 50.4 & 59.7 & 61.0 & 45.8 & 43.4 & 70.3 & 63.9 & 52.4 & 76.8 & 58.3 \\
        DANN+AutoDIAL & 51.1 & 61.4 & 71.6 & 48.0 & 58.0 & 60.2 & 48.5 & 44.3 & 70.9 & 63.1 & 50.7 & 78.0 & 58.8 \\
        DANN+DSBN & 42.9 & 59.7 & 68.4 & 47.5 & 58.9 & 59.3 & 44.5 & 36.6 & 69.6 & 56.7 & 44.4 & 69.5 & 54.8 \\
        DANN+TN & 43.5 & 60.9 & 72.1 & 51.0 & 61.5 & 62.5 & 49.6 & 46.8 & 70.4 & 63.7 & 52.2 & 77.9 & 59.3 \\
        DANN+RN & \textbf{47.3} & \textbf{63.1} & \textbf{74.4} & \textbf{57.1} & \textbf{64.7} & \textbf{68.4} & \textbf{55.2} & \textbf{47.8} & \textbf{75.9} & \textbf{68.9} & \textbf{53.5} & \textbf{79.3} & \textbf{63.0} \\
        \midrule
        CDAN(+BN) & 50.7 & 70.6 & 76.0 & 57.6 & 70.0 & 70.0 & 57.4 & 50.9 & 77.3 & 70.9 & 56.7 & 81.6 & 65.8 \\
        CDAN+AutoDIAL & 49.8 & 69.8 & 76.2 & 59.6 & 70.4 & 69.2 & 57.6 & 51.8 & 76.0 & 71.2 & 57.5 & 81.4 & 65.9 \\
        CDAN+DSBN & 47.5 & 72.6 & 76.5 & 57.0 & 68.3 & 70.0 & 58.3 & 37.7 & 78.4 & 70.2 & 51.4 & 78.4 & 64.7 \\
        CDAN+TN & 50.2 & 71.4 & 77.4 & 59.3 & 72.7 & 73.1 & 61.0 & 53.1 & 79.5 & 71.9 & 59.0 & 82.9 & 67.6 \\
        CDAN+RN & \textbf{55.6} & \textbf{72.6} & \textbf{78.1} & \textbf{65.7} & \textbf{74.7} & \textbf{74.5} & \textbf{66.2} & \textbf{57.1} & \textbf{82.0} & \textbf{75.2} & \textbf{60.5} & \textbf{84.6} & \textbf{70.6} \\
        % @ 200729, PDA later
        \bottomrule
    \end{tabular}
    } % setlength
    } % footnotesize
    \vspace{-3mm}
\end{table*}

==> latex/tabs/Supplement_Visda.tex <==
%% without reference
\begin{table*}
    \centering
    % \setlength{\abovecaptionskip}{0pt}
    % \captionsetup{font={footnotesize}}
    \footnotesize{
    % \setlength{\tabcolsep}{1.7mm}{
    \caption{The Detailed class-wise accuracy (\%) on VisDA-C.}
    \label{subtab:ResultsOnVisDA2017}
    \begin{tabular}{lccccccccccccc}
        \toprule
        % \textbf{ResNet-101} & \rotatebox{90}{aeroplane} & \rotatebox{90}{bicycle} & \rotatebox{90}{bus} & \rotatebox{90}{car} & \rotatebox{90}{horse} & \rotatebox{90}{knife} & \rotatebox{90}{motorcycle} & \rotatebox{90}{person} & \rotatebox{90}{plant} & \rotatebox{90}{skateboard} & \rotatebox{90}{train} & \rotatebox{90}{truck} & AVG \\
        \textbf{ResNet-101} & aero. & bike & bus & car & horse & knife & motor. & person & plant & sktb. & train & truck & AVG \\
        \midrule
        source only & 55.1 & 53.3 & 61.9 & 59.1 & 80.6 & 17.9 & 79.7 & 31.2 & 81.0 & 26.5 & 73.5 & 8.5 & 52.4 \\
        \midrule
        DANN(+BN) & 81.9 & 77.7 & \textbf{82.8} & 44.3 & 81.2 & 29.5 & 65.1 & 28.6 & 51.9 & \textbf{54.6} & \textbf{82.8} & 7.8 & 57.4 \\
        DANN+AutoDIAL & 86.5 & \textbf{94.4} & 61.8 & 74.3 & 95.5 & 25.9 & 59.9 & 62.3 & 80.0 & 28.7 & 71.6 & 35.9 & 64.7 \\
        DANN+DSBN & 84.0 & 83.9 & 72.0 & 75.8 & 95.2 & \textbf{61.6} & 44.8 & 60.8 & 91.4 & 41.2 & 76.3 & 48.5 & 69.6 \\
        % +TN &  &  &  &  &  &  &  &  &  &  &  &  &  \\
        DANN+RN & \textbf{90.4} & 92.7 & 71.9 & \textbf{84.5} & \textbf{96.6} & 30.2 & \textbf{81.4} & \textbf{67.9} & \textbf{95.0} & 49.2 & 73.9 & \textbf{64.8} & \textbf{74.9} \\
        \midrule
        CDAN(+BN) & 85.2 & 66.9 & \textbf{83.0} & 50.8 & 84.2 & \textbf{74.9} & \textbf{88.1} & 74.5 & 83.4 & 76.0 & 81.9 & 38.0 & 73.9 \\
        DANN+AutoDIAL & 92.8 & 94.8 & 66.5 & 74.3 & 92.4 & 51.8 & 68.3 & 60.7 & 88.4 & 54.9 & \textbf{85.4} & 61.2 & 74.5 \\
        DANN+DSBN & 88.2 & 91.0 & 79.3 & \textbf{85.5} & 93.7 & 70.7 & 57.2 & \textbf{74.2} & 91.7 & 78.0 & 81.4 & 52.3 & 78.6 \\
        % +TN &  &  &  &  &  &  &  &  &  &  &  &  &  \\
        DANN+RN & 96.7 & 94.3 & 70.4 & 84.4 & \textbf{96.6} & 36.4 & 81.8 & 68.9 & 95.4 & 81.5 & 77.9 & 77.0 & \textbf{80.1} \\
        % CDAN+RN$^\star$ & \textbf{97.8} & \textbf{97.6} & 63.4 & 74.2 & 96.4 & 23.5 & 70.4 & 72.7 & \textbf{97.4} & \textbf{89.6} & 83.0 & \textbf{94.0} & 80.0 \\
        % \midrule
        % \textbf{ResNet-50} & aeroplane & bicycle & bus & car & horse & knife & motorcycle & person & plant & skateboard & train & truck & AVG \\
        % \midrule
        % source-only &  &  &  &  &  &  &  &  &  &  &  &  &  \\
        % \midrule
        % CDAN(+BN) &  &  &  &  &  &  &  &  &  &  &  &  &  \\
        % CDAN+AutoDIAL &  &  &  &  &  &  &  &  &  &  &  &  &  \\
        % CDAN+DSBN &  &  &  &  &  &  &  &  &  &  &  &  &  \\
        % CDAN+TN &  &  &  &  &  &  &  &  &  &  &  &  &  \\
        % CDAN+RN & 96.6 & 92.5& 77.5 & 81.2 & 94.6 & 26.6 & 84.2 & 64.1 & 94.6 & 83.8 & 81.0 & 84.9 &  79.6\\
        % CDAN+RN$^\star$ & 95.6 & 97.7 & 56.9 & 75.6 & 96.4 & 21.8 & 75.8 & 67.5 & 95.2 & 76.2 & 82.2  & 90.3 & 75.6 \\
        \bottomrule
    \end{tabular}
    % } % setlength
    } % footnotesize
    \vspace{-2mm}
\end{table*}

==> latex/tabs/Supplement_alblation.tex <==
\begin{table*}
    \centering
    % \setlength{\abovecaptionskip}{0pt}
    % \captionsetup{font={footnotesize}}
    \footnotesize{
    \setlength{\tabcolsep}{1.7mm}{
    \caption{Ablation study results of RC and RA-Gate with CDAN~\cite{long2018CDAN} on Office-Home benchmark.}
    \label{subtab:ablation_RCRA_OfficeHome}
    \begin{tabular}{cc|ccccccccccccc}
        \toprule
        RC & RA & Ar$\to$Cl & Ar$\to$Pr & Ar$\to$Rw & Cl$\to$Ar & Cl$\to$Pr & Cl$\to$Rw & Pr$\to$Ar & Pr$\to$Cl & Pr$\to$Rw & Rw$\to$Ar & Rw$\to$Cl & Rw$\to$Pr & AVG \\
        \midrule
        - & - & 50.7 & 70.6 & 76.0 & 57.6 & 70.0 & 70.0 & 57.4 & 50.9 & 77.3 & 70.9 & 56.7 & 81.6 & 65.8 \\
        - & \checkmark &  52.7 & 71.6 & 77.6 & 62.1 & 72.8 & 73.4 & 62.9 & 53.2 & 80.3 & 75.1 & 59.2 & 83.2 & 68.9 \\
        %  & \checkmark & 47.5 & 72.6 & 76.5 & 57.0 & 68.3 & 70.0 & 58.3 & 37.7 & 78.4 & 70.2 & 51.4 & 78.4 & 64.7 \\
        \checkmark & \checkmark & \textbf{55.6} & \textbf{72.6} & \textbf{78.1} & \textbf{65.7} & \textbf{74.7} & \textbf{74.5} & \textbf{66.2} & \textbf{57.1} & \textbf{82.0} & \textbf{75.2} & \textbf{60.5} & \textbf{84.6} & \textbf{70.6} \\
        % @ 200729, PDA later
        \bottomrule
    \end{tabular}
    } % setlength
    } % footnotesize
    \vspace{-4mm}
\end{table*}

==> latex/tabs/Supplement_layers_ablation.tex <==
% \begin{table*}
%     \centering
%     \caption{Accuracy ($\%$) and test time comparisons.}
%     \label{spptab:test_time}
%     \footnotesize{
%     \setlength{\tabcolsep}{1.8mm}{
%     \begin{tabular}{|l|c|c|c|c|c|}
%         \toprule
%         \multicolumn{6}{|c|}{\textbf{VisDA-2017}} \\
%         \hline
%         Method & \tabincell{c}{CDAN+BN \\ ~\cite{long2018CDAN}} & \tabincell{c}{CDAN+AutoDIAL \\ ~\cite{cariucci2017autodial}} & \tabincell{c}{CDAN+TN \\ ~\cite{wang2019TN}} & \tabincell{c}{CDAN+DSBN \\ ~\cite{chang2019domain}} & \tabincell{c}{CDAN+RN \\ (Ours)} \\
%         \hline
%         Accuracy (\%) & 70.0 & 71.8 & 71.4 & 72.9 & 79.0 \\
%         \hline
%         Time (s) & 67.0536 & 101.7924 & 693.4725 & 81.9907 & 67.0536 \\
%         \hline
%         \hline
%         \multicolumn{6}{|c|}{\textbf{Office-Home: P $\to$ R}} \\
%         \hline
%         Accuracy (\%) & 77.3 & 76.0 & 79.5 & 78.4 & 82.0 \\
%         \hline
%         Time (s) &  &  &  &  &  \\
%         \bottomrule
%     \end{tabular}
%     }
%     }
% \end{table*}

% \begin{table*}
%     \centering
%     \setlength{\abovecaptionskip}{0pt}
%     \caption{Ablation study of RN on different intermediate layers. Experiments are conducted with CDAN (UDA) on $4$ randomly selected transfer tasks from Office-Home (ResNet-50). The random seed is \textit{2021}.}
%     \label{subtab:AblationOnEachLayer}
%     \small{
%     \setlength{\tabcolsep}{2.4mm}{
%     \begin{tabular}{l|cccccccc}
%         \toprule
%         Setting & BN & Layer 1 & Layer 2 & Layer 3 & Layer 4 & Layer 3,4 & Layer 2,3,4 & All Layers \\
%         \hline
%         A$\to$C & 50.7 & 50.7 & 51.2 & 52.3 & 52.5 & 56.0 & 56.1 & \textbf{56.2} \\
%         C$\to$P & 70.0 & x & 72.2 & x & 72.1 & 72.3 & 72.0 & \textbf{74.7} \\
%         P$\to$C & 50.9 & x & 54.3 & x & 54.8 & 54.6 & 54.7 & x \\
%         R$\to$A & 70.9 & x & x & x & x & x & x & x \\
%         \bottomrule
%     \end{tabular}
%     }
%     }
% \end{table*}

\begin{table}
    \centering
    % \setlength{\abovecaptionskip}{0pt}
    \caption{Ablation study of RN on different intermediate layers. Experiments are conducted with CDAN (UDA) on $3$ randomly selected transfer tasks from Office-Home (ResNet-50). 
    %The random seed is \textit{2021}.
    }
    \label{subtab:AblationOnEachLayer}
    \footnotesize{
    \setlength{\tabcolsep}{1.8mm}{
    \begin{tabular}{cccc||ccc}
        \toprule
        \multicolumn{4}{c||}{layer configuration} & \multicolumn{3}{c}{transfer task} \\
        Layer 1 & Layer 2 & Layer 3 & Layer 4 & A$\to$C & C$\to$P & A$\to$R \\
        \hline
       \checkmark  &  &  &                       & 50.7 & 72.7 &  77.6 \\
         & \checkmark  &  &                       & 51.2 & 72.2 &  77.3 \\
         &  & \checkmark  &                       & 52.3 & 72.7 &  77.4 \\
         &  &  & \checkmark                       & 52.5 & 72.1 &  77.7 \\
         &  & \checkmark  & \checkmark               & 56.0 & 72.3 &  77.7 \\
         & \checkmark  & \checkmark  & \checkmark         & 56.1 & 73.6 &  77.9 \\
        \checkmark  & \checkmark  & \checkmark  & \checkmark  & 56.2 & 74.7 &  78.1 \\
        \bottomrule
    \end{tabular}
    }
    }
\end{table}

==> latex/tabs/teaser_table.tex <==
%%% without reference
\begin{table}
% \setlength{\abovecaptionskip}{0pt}
% \setlength{\belowcaptionskip}{0pt}
    \centering
    % \captionsetup{font={footnotesize}}
    \caption{Classification accuracies ($\%$) of different normalization methods on three domain adaptation benchmarks for UDA.}
    \label{tab:teaser}
    \small{
    \setlength{\tabcolsep}{0.4mm}{
    \begin{tabular}{l|c|c|c}
        \toprule
        Method & \footnotesize{ImageCLEF-DA} & \footnotesize{VisDA-2017} & \footnotesize{Office-Home} \\
        \hline
        DANN(+BN)~\cite{ganin2015DANN} & 85.0 & 54.9 & 58.3 \\
        DANN+AutoDIAL~\cite{cariucci2017autodial} & 86.9 & 62.5 & 58.8 \\
        DANN+DSBN~\cite{chang2019domain} & 86.1 & 65.0 & 54.8\\
        DANN+TN~\cite{wang2019TN} & 87.0 & 66.3 & 59.3 \\
        DANN+RN & \textbf{88.0} & \textbf{71.4} & \textbf{63.0} \\ 
        \hline
        \hline
        CDAN(+BN)~\cite{long2018CDAN} & 87.7 & 70.0 & 65.8 \\
        CDAN+AutoDIAL~\cite{cariucci2017autodial} & 88.0 & 71.8 & 67.4 \\
        CDAN+DSBN~\cite{chang2019domain} & 86.9 & 72.9 & 64.1 \\
        CDAN+TN~\cite{wang2019TN} & 88.5 & 71.4 & 67.6 \\
        CDAN+RN & \textbf{89.2} & \textbf{79.6} & \textbf{70.6} \\
        \bottomrule
    \end{tabular}
    }
    }
    \vspace{-3mm}
\end{table}
